Z-SASLM: Zero-Shot Style-Aligned SLI Blending Latent Manipulation

We introduce Z-SASLM, a Zero-Shot Style-Aligned SLI (Spherical Linear Interpolation) Blending Latent Manipulation pipeline that overcomes the limitations of current multi-style blending methods. Conventional approaches rely on linear blending, assuming a flat latent space leading to suboptimal results when integrating multiple reference styles. In contrast, our framework leverages the non-linear geometry of the latent space by using SLI Blending to combine weighted style representations. By interpolating along the geodesic on the hypersphere, Z-SASLM preserves the intrinsic structure of the latent space, ensuring high-fidelity and coherent blending of diverse styles - all without the need for fine-tuning. We further propose a new metric, Weighted Multi-Style DINO ViT-B/8, designed to quantitatively evaluate the consistency of the blended styles. While our primary focus is on the theoretical and practical advantages of SLI Blending for style manipulation, we also demonstrate its effectiveness in a multi-modal content fusion setting through comprehensive experimental studies. Experimental results show that Z-SASLM achieves enhanced and robust style alignment. The implementation code can be found at: https://github.com/alessioborgi/Z-SASLM.

==> sec/3.2_LLMs_Based_Multi-Modal_Context_Awareness.tex <==
\subsection{Multi-Modal Content Fusion}
\label{subsec:multimodalcontentawareness}

To overcome the restriction of relying solely on text-based content inputs, in Z-SAMB \cref{architecture}, we propose a novel Multi-Modal Content Fusion Pipeline, which integrates multiple sources of content beyond text, such as images, audio, music, and real-time weather data. These modalities are conveyed into a textual form, which is then given to an LLM-based rephrasing step whose output will then be fed to the Text Encoding as positive conditioning text. More, in particular, we have:

\begin{itemize}
    \item \textbf{Image-to-Text (Img2Text) via BLIP-1}: To convey visual information, we utilize BLIP-1 (Bootstrapping Language-Image Pretraining) \cite{blip}. This model takes an image as input and generates a descriptive caption.
    
    \item \textbf{Audio-to-Text (Audio2Text) via Whisper}: Audio descriptions are processed through Whisper \cite{whisper}, a model for speech recognition and transcription.
    
    \item \textbf{Music-to-Text (Music2Text) via CLAP}: To incorporate musical information, we use Contrastive Language-Audio Pretraining (CLAP) \cite{clap}, a model linking audio data with text descriptions. CLAP extracts a music embedding $\mathbf{a} \in \mathbb{R}^d$ representing the music’s features. This embedding is compared to a set of predefined textual queries $\mathbf{q}_i \in \mathbb{R}^d$ that describe various moods and tonal qualities, such as "dark and intense"(the full list can be found in \cite{Appendix}). After that, the Cosine Similarity (CS) between the music embedding $\mathbf{a}$ and each query embedding $\mathbf{q}_i$ is calculated (yielding a similarity score between $-1$ (dissimilar) and $1$ (identical)) as:
    \begin{equation}
        \text{CS}(\mathbf{a}, \mathbf{q}_i) = \frac{\mathbf{a} \cdot \mathbf{q}_i}{\|\mathbf{a}\|_2 \cdot \|\mathbf{q}_i\|_2} = \frac{\displaystyle\sum_{j=1}^{d} a_j q_{i,j}}{\sqrt{\displaystyle\sum_{j=1}^{d} a_j^2} \cdot \sqrt{\displaystyle\sum_{j=1}^{d} q_{i,j}^2}}
    \end{equation}
    where $\mathbf{a} \cdot \mathbf{q}_i$ represents the dot product, and $\|\mathbf{a}\|_2$ and $\|\mathbf{q}_i\|_2$ are the Euclidean norms of $\mathbf{a}$ and $\mathbf{q}_i$. By comparing all queries, we create a vector of scores across $n$ queries and then the query with the highest similarity score is selected as the best descriptor of the music track:
    \begin{equation}
        \text{best\_query} = \arg\max_{i}[\text{CS}(\mathbf{a}, \mathbf{q}_1), \dots, \text{CS}(\mathbf{a}, \mathbf{q}_n)]
    \end{equation}
    
    \item \textbf{Weather-to-Text (Weather2Text) via OpenWeather API}: A last additional modality is the integration of Weather conditions converted into text descriptions using real-time data from the OpenWeather API \cite{openweatherapi}. 
    
\end{itemize}

\subsubsection{LLM-based Prompt Rephrasing}

Once textual descriptions are generated from each modality, they are concatenated into a unified textual prompt. However, simply concatenating these descriptions can result in a lengthy, unmanageable prompt, which may confuse the Text-to-Image (T2I) model. To mitigate this issue, we decided to apply a paraphrasing step based on the T5 Transformer Model \cite{t5}, fine-tuned specifically for this task. More formally, let the text descriptions from different modalities be denoted as $\mathbf{D} = [\mathbf{d}_1, \mathbf{d}_2, \dots, \mathbf{d}_n]$ where $\mathbf{d}_i$ is the description from the $i$-th modality, and $n$ represents the total number of modalities ($\leq5$ in our case). First, we concatenate the individual descriptions into a single unified text:
\begin{equation}
    \mathbf{T} = \mathbf{d}_1 + \mathbf{d}_2 + \dots + \mathbf{d}_n
\end{equation}
The summarization process is as follows:
\begin{enumerate}
    \item \textbf{Check for verbosity}: If the description $\mathbf{d}_i$ contains more than a threshold number of words, denoted as $k$ (e.g., $k = 10$), then rephrasing is performed:
    \begin{equation}
        \text{needs\_paraphrasing}(\mathbf{d}_i) = 
    \begin{cases} 
    \text{True} & \text{if } |\mathbf{d}_i| > k \\
    \text{False} & \text{otherwise}
    \end{cases}
    \end{equation}

    \item \textbf{Paraphrasing}: For each description flagged for paraphrasing, we input it into the T5 model. The model generates the paraphrased version by predicting tokens up to a maximum length $L_{\text{max}}$ and a minimum length $L_{\text{min}}$ while penalizing excessive length with a length penalty parameter $\lambda_{\text{length}}$ and where $b$ is the number of beams used in beam search:
    \begin{equation}
        \hat{\mathbf{d}}_i = \text{T5}(\mathbf{d}_i, L_{\text{max}}, L_{\text{min}}, \lambda_{\text{length}}, b)
    \end{equation}
\end{enumerate}



==> sec/experiments_old.tex <==
\section{Experiments}
\label{sec:experiments}

\subsection{Experimental Settings}
\label{subsec:experimentalsettings}

For our experimental settings, we use Stable Diffusion XL (SDXL) based on the pre-trained model \textit{`stabilityai/stable-diffusion-xl-base-1.0`} \cite{stabilityai_SDXL} to maintain consistency with Hertz \etal \cite{hertz2023StyleAligned}. However, our architecture is model-agnostic and can be adapted also to other options. The diffusion process employs a DDIM (Denoising Diffusion Implicit Models) \cite{DDIM} (scheduler settings detailed in  \cref{table:scheduler}). The Stable Diffusion XL Pipeline is initialized with parameters detailed in \cref{table:pipeline}, and optimized for mixed precision on GPUs to enhance performance.

\begin{table*}[h]
    \centering
    \caption{Weighted Multi-Style DINO VIT-B/8: Linear and SLI Blending Comparison}
    \label{tab:weighted_dino_comparison}
    \begin{tabular}{c|cccc|cccc}
        \toprule
        \textbf{Style Weights} & \multicolumn{4}{c|}{\textbf{Linear}} & \multicolumn{4}{c}{\textbf{SLI}} \\
        \midrule
        \textbf{$\{w_{\text{med}}, w_{\text{cub}}\}$} & \textbf{MS$_{\text{med}}$} & \textbf{MS$_{\text{cub}}$} & \textbf{WMS$_{\text{\scriptsize DINO-ViT-B/8}}$} & \textbf{CLIP$_{\text{score}}$} & \textbf{MS$_{\text{med}}$} & \textbf{MS$_{\text{cub}}$} & \textbf{WMS$_{\text{\scriptsize DINO-ViT-B/8}}$} & \textbf{CLIP$_{\text{score}}$}  \\
        \midrule
        $\{0, 1\}^*$       & -   & 0.47552   & 0.47552              & 0.30280 & -  & 0.47552  & 0.47552              & 0.30280\\
        $\{0.15, 0.85\}$   & 0.32466   & 0.42683   & 0.41151              & \textbf{0.31534} & 0.32595   & 0.47072  & \textbf{0.44900}     & 0.31049\\ 
        $\{0.25, 0.75\}$   & 0.35550   & 0.42250   & 0.40575              & 0.31420 & 0.33046   & 0.45447  & \textbf{0.42347}     & \textbf{0.31657}\\
        \midrule
        $\{0.5, 0.5\}$     & 0.34905   & 0.37881   & 0.36393              & 0.29232 & 0.36150   & 0.42156  & \textbf{0.39153}     & \textbf{0.31434}\\
        \midrule
        $\{0.75, 0.25\}$   & 0.35798   & 0.38327   & \textbf{0.36430}     & 0.31752 & 0.34648   & 0.35099  & 0.347601             & \textbf{0.31911}\\
        $\{0.85, 0.15\}$   & 0.35513   & 0.40860   & 0.36315              & \textbf{0.32381} & 0.36513   & 0.38286   & \textbf{0.36779}    & 0.31499\\
        $\{1, 0\}^*$       & 0.29891   & -   & 0.29891              & 0.30570 & 0.29891   & -  & 0.29891             & 0.30570\\
        \bottomrule
    \end{tabular}
    \par \vspace{0.2cm}  
    \textit{* StyleAligned \cite{hertz2023StyleAligned}, i.e., No Blending}
\end{table*}





\subsection{Weighted Multi-Style DINO VIT-B/8: Linear vs. SLI Interpolation}

We evaluate the proposed Weighted Multi-Style DINO VIT-B/8 metric to measure the alignment of generated images with multiple reference styles, comparing the two introduced blending techniques: Linear Weighted Blending and Spherical Weighted Blending (SLI). The impact on CLIP Score \cite{clip}—indicating image-text prompt alignment—is also analyzed. For consistency, we set $guidance=10$ and follow the configurations in \cref{table:scheduler} and \cref{table:pipeline} for all evaluations. With the support of ChatGPT for the input prompts creation, we have generated seven sets of nine images (the full list of prompts is provided in \cite{Appendix}). The blending weights used are {\{$\{0, 1\}$, $\{0.15, 0.85\}$, $\{0.25, 0.75\}$, $\{0.5, 0.5\}$, $\{0.75, 0.25\}$, $\{0.85, 0.15\}$, $\{1, 0\}$\}}. For each generated image, we compute the DINO-VIT metric to assess its alignment with two reference styles (Medieval and Cubism in our case), averaging results across each blending scheme for both techniques. The metrics $MS_{\text{med}}$ and $MS_{\text{cub}}$ represent the Mean Similarity for the \textit{medieval} and \textit{cubism} reference images, respectively, alongside the weighted multi-style score and CLIP score. The cases $\{0, 1\}$ and $\{1, 0\}$ reflect the baseline results of Hertz \etal \cite{hertz2023StyleAligned} (i.e., no multi-reference style blending).
\begin{figure}[h]
\centering
\includegraphics[width=\linewidth]{figures/4_Evaluations_and_Experiments/Linear_Artifacts_3Styles.png}
\caption{Linear Blending VS SLI: 3-Styles}
\label{linearartifacts}
\end{figure}
Results shown in \cref{tab:weighted_dino_comparison} indicate that SLI outperforms Linear interpolation in aligning generated images with multiple reference styles. This highlights SLI's effectiveness in navigating generative models' non-linear latent space and improving prompt-image alignment (CLIP Score) in stronger blending cases. Some SLI blending results are shown in \cref{img_slerp_bleding_medcub} and \cite{Appendix}. Notably, we can see the possibility of making a gradual style conversion if we vertically see the images. As a comment, notice that the WMS DINO ViT-B/8 score is inherently lower than its single-style counterpart. In the single-style setting, the generated image aligns well with one reference style, maximizing similarity. However, in the multi-style scenario, blending requires balancing multiple reference styles, resulting in a combined embedding that cannot fully align with any single style. This dispersion reduces the cosine similarity score, making it impossible for the multi-style score to match or exceed the single-style score due to the inherent trade-offs in style representation (More theoretical insights can be found at \cite{Appendix}). Another point to address is that we limited our evaluation to two reference styles; however, the approach is easily extendable to any number and type of reference styles, as demonstrated in \cite{Appendix}.
Experimentally, we also noticed that as the number of reference style images increases, Linear blending introduces artifacts in the generated images, unlike SLI, as shown in \cref{linearartifacts}. This is due to the assumption of a flat latent space in Linear blending.


\begin{table*}[!htb]
    \centering
    \caption{Ablation Study: Attention Scaling vs. Non-Scaling (SLI $\{0.5, 0.5\}$ Blending)}
    \label{tab:slerp_scaling_non_scaling}
    \begin{tabular}{c|ccc|cc}
        \toprule
        \textbf{Scaling Parameters (\textit{Cubism})} & \textbf{MS$_{\text{med}}$} & \textbf{MS$_{\text{cub}}$} & \(\left| \text{MS}_{\text{med}} - \text{MS}_{\text{cub}} \right|\) & \textbf{WMS$_{\text{\scriptsize DINO-ViT-B/8}}$} & \textbf{CLIP$_{\text{score}}$} \\
        \midrule
        $\{\log{(1)}, 0.125\}$      & 0.36096   & 0.40155  & 0.04059    & 0.38126               & 0.31817\\
        $\{\log{(1)}, 0.25\}$       & 0.35660   & 0.39909  & 0.04249    & 0.37784               & 0.28070\\ 
        $\{\log{(1)}, 0.5\}$        & 0.36150   & 0.42156  & 0.06006    & \textbf{0.39153}      & \textbf{0.31434}\\
        $\{\log{(1)}, 0.75\}$       & 0.36272   & 0.41224  & 0.04952    & 0.38748               & 0.31706\\
        \midrule
        $\{\log{(2)}, 1\}\dagger$   & 0.33432   & 0.45480  & 0.12048    & 0.39456               & 0.30885\\
        \bottomrule
    \end{tabular}
    \par \vspace{0.2cm}  % Adjust spacing as needed
    \textit{$\dagger$: Without Attention Scaling}
\end{table*}

\begin{table*}[t]
    \centering
    \caption{Guidance Ablation Study for SLI \{0.5, 0.5\} Blending}
    \label{tab:guidance_ablation}
    \begin{tabular}{c|ccc|cc}
        \toprule
        \multicolumn{6}{c}{\textbf{SLI \{0.5, 0.5\} Blending}} \\
        \midrule
        \textbf{Guidance} & \textbf{MS$_{\text{med}}$} & \textbf{MS$_{\text{cub}}$} & \(\left| \text{MS}_{\text{med}} - \text{MS}_{\text{cub}} \right|\) & \textbf{WMS$_{\text{\scriptsize DINO-ViT-B/8}}$} & \textbf{CLIP$_{\text{score}}$} \\
        \midrule
        5        & 0.37721   & 0.38623  & 0.00902    & 0.38172           & 0.31420\\
        10       & 0.36149   & 0.42156  & 0.06007    & 0.39153           & 0.31434\\ 
        15       & 0.35610   & 0.43315  & 0.07705    & 0.39463           & 0.31681\\
        20       & 0.38218   & 0.45844  & 0.07626    & \textbf{0.42031}  & \textbf{0.31656}\\
        25       & 0.36966   & 0.44971  & 0.08005    & 0.40968           & 0.31554\\
        30       & 0.36350   & 0.46818  & 0.10468    & 0.41584           & 0.31316\\
        \bottomrule
    \end{tabular}
    \par \vspace{0.2cm}  % Adjust this space as needed
    \textit{$\dagger$: Without Attention Scaling}
\end{table*}


\subsection{Scaling vs. Non-Scaling}

This ablation study examines the impact of different attention scaling parameters (\(\mu, \sigma\)) on SLI blending, using an equal weight configuration \(\{0.5, 0.5\}\). The study focuses on varying the scaling parameters for the more prominent style (i.e., \textit{Cubism}).
\begin{figure}[h]
\centering
\includegraphics[width=\linewidth]{figures/4_Evaluations_and_Experiments/SLERP_Scaling_vs_NonScaling.png}
\caption{Attention score rescaling's effect (SLI Blending).}
\label{img_slerp_scaling_nonscaling}
\end{figure}
The scaling parameters for \(\mu\) are set to \(\log(1)\) and \(\log(2)\), with \(\sigma\) varying from 0.125 to 1.0. The non-scaling baseline (\(\mu = \log(2)\), \(\sigma = 1\)) calculates alignment without rescaling, akin to the \textit{Medieval} setting.
As shown in \cref{tab:slerp_scaling_non_scaling}, we observe that a very crucial factor indicating the need for attention scaling is to monitor \(\left| \text{MS}_{\text{med}} - \text{MS}_{\text{cub}} \right|\) that measures the difference in mean similarity. The lower this value is, the less possibility that one style stands above the other. The non-scaling case (\(\mu = \log(2)\), \(\sigma = 1\)) shows a larger difference of 0.12048, suggesting a reduced alignment balance between the two styles. Despite these variations, the CLIP$_{\text{score}}$ remains fairly consistent across all settings. Optimal style alignment with minimal loss in WMS$_{\text{\scriptsize DINO-ViT-B/8}}$ and an improved CLIP$_{\text{score}}$ is achieved at \(\mu = \log(1)\) and \(\sigma = 0.5\). An example of the impact we have before and after the scaling step can be found in \cref{img_slerp_scaling_nonscaling}.




\subsection{SLI's Guidance Ablation}

This ablation study investigates the impact of different guidance scales on SLI blending, specifically comparing a standard guidance scale of 10 to other scales to determine their effect on the primary metrics. Results of this ablation are present in \cref{tab:guidance_ablation} and in \cite{Appendix}. From this study, we can reveal that increasing the guidance scale generally raises the WMS\textsubscript{DINO-ViT-B/8} metric. However, this comes with a higher absolute difference between mean similarities (\( \left| \text{MS}_{\text{med}} - \text{MS}_{\text{cub}} \right| \)), up to 20 Guidance, that turns out to be the best setting. This aligns with the challenges discussed in \cref{dynamic_scaling_selection} and suggests a potential correlation: as guidance increases, more pronounced attention scaling may be necessary. Further exploration of this relationship is suggested for future work. We can also see that guidance affects the structural properties of generated images, but its influence on the alignment between generated images and textual prompts (as measured by CLIP) remains minimal across this range.




\section{Conclusions}
\label{sec:conclusion}

We proposed a novel framework for multi-style blending and multi-modal content-fusion image generation, leveraging Stable Diffusion XL for consistent style alignment. Key contributions include the introduction of Multi-Reference Style Blending with Linear and SLI techniques, enabling seamless style transitions and new style creation, enhancing creative flexibility beyond single-style methods. We developed the Weighted Multi-Style DINO VIT-B/8 metric to evaluate multi-style consistency, filling a gap in current single-style evaluation metrics. Our approach maintains coherence across multiple reference styles, elevating the creative potential of diffusion models. The framework's Multi-Modal Content Fusion incorporates diverse inputs enriching image generation with contextual relevance. 
In future work, we plan to explore the implementation of linear attention mechanisms to improve computational efficiency while handling large-scale image generation tasks. 

